MambaU-Lite: A Lightweight Model based on Mamba and Integrated Channel-Spatial Attention for Skin Lesion Segmentation

Early detection of skin abnormalities plays a crucial role in diagnosing and treating skin cancer. Segmentation of affected skin regions using AI-powered devices is relatively common and supports the diagnostic process. However, achieving high performance remains a significant challenge due to the need for high-resolution images and the often unclear boundaries of individual lesions. At the same time, medical devices require segmentation models to have a small memory foot-print and low computational cost. Based on these requirements, we introduce a novel lightweight model called MambaU-Lite, which combines the strengths of Mamba and CNN architectures, featuring just over 400K parameters and a computational cost of more than 1G flops. To enhance both global context and local feature extraction, we propose the P-Mamba block, a novel component that incorporates VSS blocks along-side multiple pooling layers, enabling the model to effectively learn multiscale features and enhance segmentation performance. We evaluate the model's performance on two skin datasets, ISIC2018 and PH2, yielding promising results. Our source code will be made publicly available at: https://github.com/nqnguyen812/MambaU-Lite.

==> bibitems_full_converted1.tex <==

\bibitem{ronneberger2015u} Olaf Ronneberger, Philipp Fischer, Thomas Brox, "U-net: convolutional networks for biomedical image segmentation," \textit{}, 2015.

\bibitem{valanarasu2022unext} Jeya Maria Jose Valanarasu, Vishal M. Patel, "UNext: MLP-based rapid medical image segmentation network," \textit{International Conference on Medical Image Computing and Computer-Assisted Intervention}, 2022.

\bibitem{oktay2018attention} Ozan Oktay, Jo Schlemper, Loic Le Folgoc, Matthew Lee, Mattias Heinrich, Kazunari Misawa, Kensaku Mori, Steven McDonagh, Nils Y Hammerla, Bernhard Kainz, others, "Attention u-net: learning where to look for the pancreas," \textit{arXiv preprint arXiv:1804.03999}, 2018.

\bibitem{pham2021ear} Van-Truong Pham, Thi-Thao Tran, Pa-Chun Wang, Po-Yu Chen, Men-Tzung Lo, "EAR-UNet: A deep learning-based approach for segmentation of tympanic membranes from otoscopic images," \textit{Artificial Intelligence in Medicine}, vol. 115, pp. 102065, 2021.


\bibitem{vaswani2017attention} A Vaswani, "Attention is all you need," \textit{Advances in Neural Information Processing Systems}, 2017.


\bibitem{dosovitskiy2020image} Alexey Dosovitskiy, "An image is worth 16x16 words: transformers for image recognition at scale," \textit{arXiv preprint arXiv:2010.11929}, 2020.  



\bibitem{chen2021transunet} Jieneng Chen, Yongyi Lu, Qihang Yu, Xiangde Luo, Ehsan Adeli, Yan Wang, Le Lu, Alan L Yuille, Yuyin Zhou, "Transunet: transformers make strong encoders for medical image segmentation," \textit{arXiv preprint arXiv:2102.04306}, 2021.



\bibitem{wang2022uctransnet} Haonan Wang, Peng Cao, Jiaqi Wang, Osmar R Zaiane, "Uctransnet: rethinking the skip connections in u-net from a channel-wise perspective with transformer," \textit{}, 2022.


\bibitem{cao2022swin} Hu Cao, Yueyue Wang, Joy Chen, Dongsheng Jiang, Xiaopeng Zhang, Qi Tian, Manning Wang, "Swin-unet: unet-like pure transformer for medical image segmentation," \textit{}, 2022.


\bibitem{gu2023mamba} Albert Gu, Tri Dao, "Mamba: linear-time sequence modeling with selective state spaces," \textit{arXiv preprint arXiv:2312.00752}, 2023.

\bibitem{zhu2024vision} Lianghui Zhu, Bencheng Liao, Qian Zhang, Xinlong Wang, Wenyu Liu, Xinggang Wang, "Vision mamba: efficient visual representation learning with bidirectional state space model," \textit{arXiv preprint arXiv:2401.09417}, 2024.


\bibitem{liu2024vmambavisualstatespace} Yue Liu, Yunjie Tian, Yuzhong Zhao, Hongtian Yu, Lingxi Xie, Yaowei Wang, Qixiang Ye, Yunfan Liu, "Vmamba: visual state space model," \textit{}, 2024.


\bibitem{dinh20231m} Binh-Duong Dinh, Thanh-Thu Nguyen, Thi-Thao Tran, Van-Truong Pham, "1M parameters are enough? A lightweight CNN-based model for medical image segmentation," \textit{2023 Asia Pacific Signal and Information Processing Association Annual Summit and Conference}, pp. 1279--1284, 2023.
\bibitem{rahman2024mamba} Md Maklachur Rahman, Abdullah Aman Tutul, Ankur Nath, Lamyanba Laishram, Soon Ki Jung, Tracy Hammond, "Mamba in vision: a comprehensive survey of techniques and applications," \textit{arXiv preprint arXiv:2410.03105}, 2024.

\bibitem{heidari2024computation} Moein Heidari, Sina Ghorbani Kolahi, Sanaz Karimijafarbigloo, Bobby Azad, Afshin Bozorgpour, Soheila Hatami, Reza Azad, Ali Diba, Ulas Bagci, Dorit Merhof, others, "Computation-efficient era: a comprehensive survey of state space models in medical image analysis," \textit{arXiv preprint arXiv:2406.03430}, 2024.

\bibitem{woo2018cbam} Sanghyun Woo, Jongchan Park, Joon-Young Lee, In So Kweon, "CBAM: Convolutional block attention module," \textit{Proceedings of the European Conference on Computer Vision (ECCV)}, pp. 3--19, 2018.

\bibitem{nguyen2024ac} Viet-Thanh Nguyen, Van-Truong Pham, Thi-Thao Tran, "AC-MAMBASEG: An adaptive convolution and Mamba-based architecture for enhanced skin lesion segmentation," \textit{arXiv preprint arXiv:2405.03011}, 2024.

\bibitem{le2023attention} Thanh Viet Le, Hoang-Minh-Quang Le, Van-Yem Vu, Thi-Thao Tran, Van-Truong Pham, "Attention convmixer model and application for fish species classification," \textit{EAI Endorsed Transactions on Industrial Networks and Intelligent Systems}, 2023.

\bibitem{xu2023dcsau} Qing Xu, Zhicheng Ma, HE Na, Wenting Duan, "Dcsau-net: a deeper and more compact split-attention u-net for medical image segmentation," \textit{Computers in Biology and Medicine}, 2023.











\bibitem{diakogiannis2020resunet} Foivos I Diakogiannis, Fran{\c{c}}ois Waldner, Peter Caccetta, Chen Wu, "Resunet-a: a deep learning framework for semantic segmentation of remotely sensed data," \textit{ISPRS Journal of Photogrammetry and Remote Sensing}, 2020.




\bibitem{hou2022vision} Qibin Hou, Zihang Jiang, Li Yuan, Ming-Ming Cheng, Shuicheng Yan, Jiashi Feng, "Vision permutator: a permutable mlp-like architecture for visual recognition," \textit{IEEE transactions on pattern analysis and machine intelligence}, 2022.


\bibitem{zhou2018unet++} Zongwei Zhou, Md Mahfuzur Rahman Siddiquee, Nima Tajbakhsh, Jianming Liang, "Unet++: a nested u-net architecture for medical image segmentation," \textit{}, 2018.

\bibitem{huang2020unet} Huimin Huang, Lanfen Lin, Ruofeng Tong, Hongjie Hu, Qiaowei Zhang, Yutaro Iwamoto, Xianhua Han, Yen-Wei Chen, Jian Wu, "Unet 3+: a full-scale connected unet for medical image segmentation," \textit{}, 2020.

\bibitem{milletari2016v} Fausto Milletari, Nassir Navab, Seyed-Ahmad Ahmadi, "V-net: fully convolutional neural networks for volumetric medical image segmentation," \textit{}, 2016.

\bibitem{fan2020ma} Tongle Fan, Guanglei Wang, Yan Li, Hongrui Wang, "Ma-net: a multi-scale attention network for liver and tumor segmentation," \textit{IEEE Access}, 2020.





